UniSumEval: Towards Unified, Fine-Grained, Multi-Dimensional Summarization Evaluation for LLMs

Existing benchmarks for summarization quality evaluation often lack diverse input scenarios, focus on narrowly defined dimensions (e.g., faithfulness), and struggle with subjective and coarse-grained annotation schemes. To address these shortcomings, we create UniSumEval benchmark, which extends the range of input context (e.g., domain, length) and provides fine-grained, multi-dimensional annotations. We use AI assistance in data creation, identifying potentially hallucinogenic input texts, and also helping human annotators reduce the difficulty of fine-grained annotation tasks. With UniSumEval, we benchmark nine latest language models as summarizers, offering insights into their performance across varying input contexts and evaluation dimensions. Furthermore, we conduct a thorough comparison of SOTA automated summary evaluators. Our benchmark data will be available at https://github.com/DISL-Lab/UniSumEval-v1.0.

==> tables/IAA/alignment_IAA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{cccc}
\Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{Length}} 
& 
\multirow{3}{*}{\textbf{Dataset}}
& 
\multicolumn{2}{c}{\centering \textbf{IAA}}                                                                          \\ \cmidrule(l){3-4} 
                                 &                                   & \makecell{
                                 \textbf{Keyfact-level} 
                                 } & 
                                 \makecell{
                                 \textbf{Sentence-level}
                                 } 
\\ \cmidrule(){1-4}
\multirow{4}{*}{Short}           
& CNNDM                             & 0.41                                   & 0.50                                                                                     \\
& WikiHow                           & 0.51                                   & 0.62                                                    \\
& MultiWOZ                          & 0.47                                    & 0.59                                                   \\
& MultiWOZ\_RED                          & 0.45                                    & 0.49                                                   \\
& DialogSum                         & 0.51                                    & 0.49                                                   \\ 
\cmidrule(){1-4}
\multirow{5}{*}{Long}            
& PubMed                            & 0.35                                    & 0.45                               \\
 & GovReport                         & 0.37                                    & 0.33                           \\
 & SQuALITY                          & 0.31                                    & 0.30                           \\
 & MediaSum                          & 0.42                                    & 0.53                           \\
 & MeetingBank                       & 0.43                                    & 0.52                           \\
\cmidrule(){1-4}
                                \multicolumn{2}{c}{Avg. IAA}          & \multicolumn{1}{c}{0.42}                & \multicolumn{1}{c}{0.48}  \\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
\end{center}
\caption{Statistics of and the IAA of keyfact alignment annotation across ten datasets. }
\label{tab:hallu_iaa_table}
\end{table}

==> tables/IAA/hallu_IAA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{cccc}
\Xhline{3\arrayrulewidth}
\multirow{4}{*}{\textbf{Length}} 
& 
\multirow{4}{*}{\textbf{Dataset}}
& 
\multicolumn{2}{c}{\centering \textbf{IAA}}                                                                          \\ \cmidrule(l){3-4} 
                                 &                                   & \makecell{
                                 \textbf{Between} \\ \textbf{Machine} \\
                                 \textbf{\& Humans}
                                 } & 
                                 \makecell{
                                 \textbf{Among} \\ \textbf{Humans}
                                 } 
\\ \cmidrule(){1-4}
\multirow{5}{*}{Short}           & CNNDM                             & 0.91                                    & 0.63                       \multirow{4}{*}{}        \\
                                 & WikiHow                           & 0.96                                    & 0.78                                                    \\
                                 & MultiWOZ                          & 0.86                                    & 0.66                                                    \\
                                 & MultiWOZ\_RED                          & 0.84                                    & 0.68                                                    \\
                                 & DialogSum                         & 0.92                                    & 0.78                                                    \\ 
\cmidrule(){1-4}
\multirow{5}{*}{Long}            & PubMed                            & 0.82                                    & 0.42                       \multirow{5}{*}{}        \\
                                 & GovReport                         & 0.74                                    & 0.49                           \\
                                 & SQuALITY                          & 0.83                                    & 0.48                           \\
                                 & MediaSum                          & 0.86                                    & 0.43                           \\
                                 & MeetingBank                       & 0.92                                    & 0.54                           \\
\cmidrule(){1-4}
                                \multicolumn{2}{c}{Avg. IAA}          & \multicolumn{1}{c}{0.87}                & \multicolumn{1}{c}{0.59}  \\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
\end{center}
\caption{Statistics of and the inter-annotator agreement (IAA) of faithfulness annotation across ten datasets. "Between Machine \& Humans" refers to the IAA (Cohen's Kappa \cite{}) between the machine labels we provided and the majority class of the three annotators. "Among Humans" stands on the IAA (Krippendorff's alpha\cite{}) among the three annotators.}
\label{tab:hallu_iaa_table}
\end{table}

==> tables/IAA/iaa_improvement_table.tex <==
\begin{comment}
\begin{table}[h!]
\footnotesize
\centering
{%
\begin{tabular}{cc}
\toprule
Applied Methods & IAA \\ \hline
Cont. Map & 0.28 \\
\multicolumn{1}{c}{Cont. Map + MBR (w.o explanation)} & 0.55 \\
\multicolumn{1}{c}{Cont. Map + MBR (with explanation)} & 0.63 \\ 
\bottomrule
\end{tabular}%
}
\vspace*{-0.25cm}
\caption{IAA Improvement with AI-assisted fact verification in the news domain. Cont.Map: Contextual mapping; MBR: Machine-based reasoning.}
\label{tab:IAA_improvement}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[t!]
\begin{center}
\footnotesize
\begin{tabular}{L{3.5cm} X{0.8cm} X{2.1cm} } \toprule
AI-assistance & IAA & \!\!Disagreement\!\! \\\midrule
\!\!Contextual mapping\!\!            & 0.28 & - \\
\!\!~~+ machine-based labeling\!\!    & 0.55 & - \\
\!\!~~+ machine-based reasoning\!\!   & 0.63 & (18.7\%, 2.55\%) \\\bottomrule
\end{tabular}
\end{center}
\end{table}
\end{comment}


% \begin{table}[h!]
% \footnotesize
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cc}
% \toprule
% \textbf{Applied Methods} & \textbf{IAA} \\ \hline
% Cont. Map & 0.28 \\
% \multicolumn{1}{c}{Cont. Map + MBR (w.o explanation)} & 0.55 \\
% \multicolumn{1}{c}{Cont. Map + MBR (with explanation)} & 0.63 \\ 
% \bottomrule
% \end{tabular}%
% }
% \captionsetup{skip=0.1cm}
% \caption{IAA Improvement with AI-assisted fact verification in the news domain. Cont.Map: Contextual mapping; MBR: Machine-based reasoning.}
% \label{tab:IAA_improvement}
% \end{table}


% \begin{table}[]
% \footnotesize
% \vspace*{-0.05cm}
% \begin{tabular}{cc}
% \toprule
% Applied Methods & IAA \\ \hline
% Cont. Map* & 0.28 \\
% \multicolumn{1}{c}{Cont. Map + MBR** (w.o explanation)} & 0.55 \\
% \multicolumn{1}{c}{Cont. Map + MBR (with explanation)} & 0.63 \\ 
% \bottomrule
% \end{tabular}
% % \vspace*{-0.25cm}
% \caption{IAA Improvement with AI-assisted fact verification in news domain. *Contextual mapping **Machine-based reasoning.}
% \label{tab:IAA_improvement}
% \end{table}







% \begin{table*}[t!]
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1}
% \begin{tabular}{ccclccccc}
% \hline
% \textbf{Stage} &
%   \textbf{Qualification} &
%   \textbf{\# of Trick} &
%   \multicolumn{1}{c}{\textbf{Description}} &
%   \textbf{\# of Doc \&   summ pair} &
%   \textbf{Reject Ratio} &
%   \textbf{Avg. Seconds} &
%   \textbf{IAA} &
%   \textbf{False   annotation Ratio} \\ \hline
% Round 1 &
%   \# of HIT \textgreater 100 &
%   - &
%   Default &
%   10 &
%   69.40\% &
%   799.5 &
%   -0.04 &
%   28.2\% \\
% Round 2 &
%   Master &
%   - &
%   + Con. Map. &
%   24 &
%   6.50\% &
%   285 &
%   0.283 &
%   3.7\% \\
% Round 3 &
%   HIT \% \textgreater 90\%, \# of   HIT \textgreater 500, Easy qual Test &
%   2 &
%   + Con. Map. + hallu.   text &
%   21 &
%   1.50\% &
%   1021.7 &
%   -0.06 &
%   13.1\% \\
% Round 4 &
%   HIT \% \textgreater 90\%, \# of   HIT \textgreater 500, Easy qual Test &
%   2 &
%   + Con. Map. + hallu.   Text + Mac. Label (Agree X) &
%   22 &
%   33.30\% &
%   847.3 &
%   0.55 &
%   26.5\% \\
% Round 5 &
%   HIT \% \textgreater 90\%, \# of   HIT \textgreater 500, Easy qual Test &
%   2 &
%   + Con. Map. + hallu.   Text + Mac. Label (Agree X) + Error Integration &
%   74 &
%   57.10\% &
%   795.4 &
%   0.01 &
%   8.0\% \\
% Round 5 &
%   HIT \% \textgreater 90\%, \# of   HIT \textgreater 500, Hard qual Test &
%   2 &
%   + Con. Map. + hallu.   Text + Mac. Label (Agree X) + Error Integration &
%   125 &
%   30.30\% &
%   684.7 &
%   0.07 &
%   8.3\% \\
% Round 6 &
%   HIT \% \textgreater 95\%, \# of   HIT \textgreater 1000, Hard qual Test &
%   2 &
%   + Con. Map. + hallu.   Text + Mac. Label (Agree O) + Error Integration &
%   136 &
%   40.40\% &
%   448 &
%   0.73 &
%   11.1\% \\
% Final (in   paper) &
%   HIT \% \textgreater 95\%, \# of   HIT \textgreater 1000, Hard qual Test &
%   2 &
%   + Con. Map. + hallu.   Text + Mac. Label (Agree O) + Error Integration &
%   212 &
%   41.40\% &
%   466.3 &
%   0.63 &
%   8.3\% \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table*}

==> tables/benchmark_evaluator/before_editing/benchmark_comp_before_editing.tex <==
\begin{table*}[t]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{
    ccccccccccccc}
\toprule
\multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
\multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% \multicolumn{10}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-12} 
% & & 
\multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
\multirow{3}{*}{\textbf{\makecell{Avg. \\ Score}}} \\ 
\cmidrule(lr){3-7}
\cmidrule(lr){8-12}
& & 
\textbf{News} & 
\textbf{Lifestyle} & 
\textbf{Report} & 
\textbf{\makecell{Med \\ lit}} & 
\textbf{Sci-fi} & 
\textbf{\makecell{Daily \\ Life}} & 
\textbf{Booking} & 
\textbf{\makecell{Booking \\ (RED)}} & 
\textbf{Interview} & 
\textbf{Meeting} & 
\\ 
\midrule
\multirow{2}{*}{Simllarity}     
& BERTScore              & 0.17 & 0.07          & 0.15  & 0.21  & 0.25 & 0.21 & -    & -     & 0.31  & 0.18  & 0.19 \\
& BARTScore              & 0.11 & -0.13         & 0.21  & 0.16  & 0.21 & 0.24 & -    & -     & 0.08  & 0.15  & 0.13 \\
\midrule
QA-Based                        
& UniEval-Rel            & 0.07 & 0.02          & 0.04  & 0.08  & 0.28 & 0.04 & -    & -     & 0.18  & 0.16  & 0.11 \\
\midrule
\multirow{2}{*}{Two-stage} 
& Lite\textsuperscript{3}Pyramid           & 0.04 & 0.06          & 0.15  & 0.21  & 0.34 & 0.18 & -    & -     & 0.11  & 0.06  & 0.14 \\
& A\textsuperscript{2}CU                   & 0.18 & 0.14          & -0.05 & -0.01 & 0.23 & 0.15 & -    & -     & -0.03 & -0.03 & 0.07 \\
\midrule
One-stage                  
& A\textsuperscript{3}CU                   & 0.00 & 0.08          & -0.04 & -0.09 & 0.22 & 0.20 & -    & -     & 0.08  & -0.01 & 0.06 \\
\midrule
\multirow{2}{*}{LLM-Based}      & GEval-Rel              & 0.12 & 0.36          & 0.17  & 0.14  & 0.49 & 0.27 & 0.17 & -0.04 & 0.45  & 0.37  & 0.25 \\
                                & G-Eval-Con & 0.21 & 0.36 & 0.16  & 0.28  & 0.46 & 0.29 & 0.01 & 0.04  & 0.45  & 0.39  & 0.27 \\
\bottomrule
\end{tabular}
\caption{Summary level Pearson correlation coefficients between conciseness score and automatic metrics scores across ten domains.}
\end{center}
\end{table*}



==> tables/benchmark_faith_dialogue_each_dataset.tex <==
\begin{table*}[]
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4.8pt}
\begin{tabular}{@{}cccccccccccc@{}}

\Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{\makecell{Type}}} & \multirow{3}{*}{\textbf{Metric}} & \multicolumn{6}{c}{\textbf{Short}} & \multicolumn{4}{c}{\textbf{Long}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-12}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{DialogSum}} & \multicolumn{2}{c}{\textbf{MultiWOZ}} & \multicolumn{2}{c}{\textbf{MultiWOZ\_RED}} & \multicolumn{2}{c}{\textbf{MediaSum}} & \multicolumn{2}{c}{\textbf{MeetingBank}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
& \multicolumn{1}{c}{} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} \\
\midrule
\multirow{5}{*}{Simllarity} &
  ROUGE-1 &
  0.04 &
  0.09 &
  - &
  - &
  - &
  - &
  0.07 &
  -0.08 &
  0.14* &
  -0.12 \\
 &
  ROUGE-2 &
  -0.03 &
  0.00 &
  - &
  - &
  - &
  - &
  0.09 &
  -0.08 &
  0.04 &
  -0.43 \\
 &
  ROUGE-L &
  0.03 &
  0.04 &
  - &
  - &
  - &
  - &
  0.08 &
  -0.10 &
  0.05 &
  -0.36 \\
 &
  BERTScore &
  0.05 &
  0.10 &
  - &
  - &
  - &
  - &
  0.16* &
  0.03 &
  0.17* &
  0.06 \\
 &
  BARTScore &
  -0.06 &
  -0.09 &
  - &
  - &
  - &
  - &
  0.21* &
  0.28 &
  -0.05 &
  -0.04 \\
\midrule
\multirow{2}{*}{QA-Based} &
  UniEval &
  0.12 &
  0.17* &
  - &
  - &
  - &
  - &
  0.17* &
  -0.22 &
  0.07 &
  -0.01 \\
 &
  QAFactEval &
  0.22* &
  0.20* &
  0.06 &
  -0.10 &
  0.06 &
  0.10 &
  -0.04 &
  -0.28 &
  0.05 &
  -0.36 \\
\midrule
\multirow{4}{*}{NLI-Based} &
  SummaC-Conv &
  -0.11 &
  -0.20* &
  -0.03 &
  -0.72* &
  -0.14* &
  -0.53 &
  -0.21* &
  -0.72* &
  -0.09 &
  -0.54 \\
 &
  NonFacts &
  0.35* &
  0.34* &
  0.12 &
  0.78* &
  0.27* &
  0.82* &
  0.07 &
  \textbf{0.80*} &
  0.19* &
  0.76* \\
 &
  AlignScore &
  0.33* &
  0.39* &
  0.12 &
  0.43 &
  0.39* &
  0.88* &
  0.09 &
  -0.35 &
  0.31* &
  0.71* \\
 &
  MiniCheck-FT &
  0.22* &
  0.24* &
  0.30* &
  0.27 &
  0.07 &
  -0.37 &
  0.15* &
  -0.22 &
  0.04 &
  -0.06 \\
\midrule
\multirow{3}{*}{LLM-Based} &
  GEval &
  \textbf{0.68*} &
  \textbf{0.63*} &
  \textbf{0.62*} &
  0.92* &
  \textbf{0.71*} &
  \textbf{1.0*} &
  0.48* &
  0.68* &
  \textbf{0.58*} &
  \textbf{0.87*} \\
 &
  GEval-Sen &
  0.46* &
  0.53* &
  0.59* &
  \textbf{0.93*} &
  0.55* &
  0.98* &
  \textbf{0.52*} &
  0.55 &
  0.52* &
  0.77* \\
 &
  FactScore &
  -0.06 &
  -0.05 &
  -0.13 &
  0.12 &
  0.56* &
  0.88* &
  0.10 &
  0.23 &
  0.08 &
  0.51 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Summary level Pearson correlation and system level Spearman rank correlation coefficients between human annotations and metrics scores in dialogue dataset. Best results on each domain are in \textbf{bold}. * indicates p-value < 0.05. 나중에 시간날 때 값 다 맞춰보기}
\end{table*}



==> tables/benchmark_faith_non_dialogue_each_dataset.tex <==
\begin{table*}[]
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4.8pt}
\begin{tabular}{@{}cccccccccccc@{}}
\Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{\makecell{Type}}} & \multirow{3}{*}{\textbf{Metric}} & \multicolumn{4}{c}{\textbf{Short}} & \multicolumn{6}{c}{\textbf{Long}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-12}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{CNNDM}} & \multicolumn{2}{c}{\textbf{WikiHow}} & \multicolumn{2}{c}{\textbf{GovReport}} & \multicolumn{2}{c}{\textbf{PubMed}} & \multicolumn{2}{c}{\textbf{SQuALITY}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
& \multicolumn{1}{c}{} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} & \textbf{Summ.} & \textbf{Sys.} \\
\midrule
\multirow{5}{*}{Simllarity} &
  ROUGE-1 &
  0.12 &
  -0.13 &
  0.08 &
  0.16 &
  0.27* &
  0.19 &
  0.30* &
  0.58 &
  0.18* &
  0.73* \\
 &
  ROUGE-2 &
  0.06 &
  -0.25 &
  0.04 &
  0.20 &
  0.21* &
  0.26 &
  0.20* &
  0.58 &
  0.20* &
  0.67* \\
 &
  ROUGE-L &
  0.05 &
  -0.32 &
  0.08 &
  0.26 &
  0.22* &
  0.21 &
  0.26* &
  0.62 &
  0.16* &
  0.72* \\
 &
  BERTScore &
  0.10 &
  -0.23 &
  0.10 &
  0.16 &
  0.29* &
  0.11 &
  0.25* &
  0.55 &
  0.03 &
  0.48 \\
 &
  BARTScore &
  -0.17* &
  -0.75* &
  -0.15* &
  -0.55 &
  -0.19* &
  -0.65 &
  0.13 &
  -0.17 &
  0.03 &
  0.18 \\
\midrule
\multirow{2}{*}{QA-Based} &
  UniEval &
  0.11 &
  -0.52 &
  0.54* &
  0.74* &
  -0.22* &
  -0.60 &
  -0.09 &
  -0.83* &
  -0.26* &
  -0.68* \\
 &
  QAFactEval &
  0.14* &
  -0.73* &
  0.45* &
  0.07 &
  -0.07 &
  -0.79* &
  0.19* &
  0.03 &
  -0.15* &
  -0.72* \\
\midrule
\multirow{4}{*}{NLI-Based} &
  SummaC-Conv &
  0.07 &
  -0.73* &
  0.14* &
  0.25 &
  -0.15* &
  -0.44 &
  -0.13 &
  -0.43 &
  -0.08 &
  -0.67* \\
 &
  NonFacts &
  0.34* &
  0.62 &
  0.29* &
  0.29 &
  0.02 &
  0.17 &
  0.50* &
  \textbf{0.70*} &
  0.22* &
  0.91* \\
 &
  AlignScore &
  0.18* &
  -0.40 &
  0.32* &
  0.24 &
  0.17* &
  -0.28 &
  0.09 &
  -0.10 &
  0.26* &
  0.45 \\
 &
  MiniCheck-FT &
  0.24* &
  -0.37 &
  0.69* &
  0.71* &
  -0.02 &
  -0.31 &
  0.13 &
  -0.47 &
  -0.10 &
  -0.90* \\
\midrule
\multirow{3}{*}{LLM-Based} &
  GEval &
  \textbf{0.65*} &
  \textbf{0.93*} &
  \textbf{0.72*} &
  \textbf{0.78*} &
  0.41* &
  \textbf{0.55} &
  -0.14 &
  0.32 &
  \textbf{0.42*} &
  \textbf{0.93*} \\
 &
  GEval-Sen &
  0.63* &
  0.78* &
  0.57* &
  0.75* &
  \textbf{0.47*} &
  0.37 &
  \textbf{0.55*} &
  0.68* &
  0.39* &
  0.90* \\
 &
  FactScore &
  0.07 &
  0.13 &
  -0.02 &
  -0.01 &
  -0.11 &
  -0.08 &
  0.10 &
  -0.10 &
  -0.00 &
  -0.43 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Summary level Pearson correlation and system level Spearman rank correlation coefficients between human annotations and metrics scores in non-dialogue dataset. Best results on each domain are in \textbf{bold}. * indicates p-value < 0.05. . 나중에 시간날 때 값 다 맞춰보기}
\end{table*}




==> tables/benchmarks_comparison.tex <==
% \begin{table}[]
% \footnotesize
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|l|ccc|ccc|cc|}
% \hline
% \multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{Input Diversity} & \multicolumn{3}{c|}{Annotation Scheme} & \multicolumn{2}{c|}{Data Generation} \\ \hline
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\# of \\ Domains\end{tabular}} & \multicolumn{1}{c|}{Format} & \begin{tabular}[c]{@{}c@{}}Length \\ (Min, Max)\end{tabular} & \multicolumn{1}{c|}{Granuality} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Evaluation\\  Dimensions\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Measurement\\ Objectiveness\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}LLM-genearted \\ Summaries\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Error\\ Source\end{tabular} \\ \hline
% SummEval & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Non-dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Coarse-grained \\ (Summary)\end{tabular}} & \multicolumn{1}{c|}{Multiple} & Subjective & \multicolumn{1}{c|}{No} & Real \\ \hline
% FRANK & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Non-dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Fine-grained \\ (Sentence)\end{tabular}} & \multicolumn{1}{c|}{Single} & Objective & \multicolumn{1}{c|}{No} &  \\ \hline
% SummaC & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Non-dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{No} &  \\ \hline
% AFACT & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Non-dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{No} &  \\ \hline
% LongEval & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Coarse-grained \\ (Summary)\end{tabular}} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{No} &  \\ \hline
% DIALSUMEVAL & \multicolumn{1}{c|}{Single} & \multicolumn{1}{c|}{Dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Coarse-grained \\ (Summary)\end{tabular}} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{No} &  \\ \hline
% DIALSUMFACT & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{Dialouge} & \begin{tabular}[c]{@{}c@{}}Mixed \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Fine-grained \\ (Sentence)\end{tabular}} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{No} &  \\ \hline
% SUMMEDITS & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{Non-dialouge} & \begin{tabular}[c]{@{}c@{}}Short \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Coarse-grained \\ (Summary)\end{tabular}} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{Yes} & Synthetic \\ \hline
% TOFUEVAL & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{Dialouge} & \begin{tabular}[c]{@{}c@{}}Mixed \\ ()\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mixed \\ (Sentence \&amp; \\ Summary)\end{tabular}} & \multicolumn{1}{c|}{Multiple} & Subjective & \multicolumn{1}{c|}{Yes} & Real \\ \hline
% CSEVAL & \multicolumn{1}{c|}{Mixed} & \multicolumn{1}{c|}{Both} & Mixed ( ) & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Fine-grained \\ (Sentence \&amp; \\ Key Fact)\end{tabular}} & \multicolumn{1}{c|}{Multiple} & Objective & \multicolumn{1}{c|}{Yes} & Real \\ \hline
% \end{tabular}
% \caption{벤치마크 비교 테이블, 나중에 업데이트 예정}
% \end{table}

==> tables/comprehensive_evaluation_results_multi_table_.tex <==
% \begin{table*}[!h]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{
%     ccccccccccccc}
% \toprule
% \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{4}{c}{\textbf{Dialogue}} & 
% \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% \multirow{3}{*}{\makecell{\textbf{DoS}}} \\  
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-11}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{\makecell{Med \\ lit}} & 
% \textbf{Sci-fi} & 
% \textbf{\makecell{Daliylife}} & 
% \textbf{Booking} & 
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}} &
%   BART\textsubscript{large} &
%   91.5 &
%   83.7 &
%   91.0 &
%   91.9 &
%   85.7 &
%   80.3 &
%   82.8 &
%   81.1 &
%   74.7 &
%   84.2 &
%   17.2 \\
%  &
%   Flan-T5\textsubscript{large} &
%   84.7 &
%   96.0 &
%   85.3 &
%   90.0 &
%   74.7 &
%   66.0 &
%   78.6 &
%   89.5 &
%   61.4 &
%   80.2 &
%   34.6 \\
% \midrule
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   81.8 &
%   62.8 &
%   \textbf{100.0} &
%   75.8 &
%   77.6 &
%   83.6 &
%   90.0 &
%   81.1 &
%   81.3 &
%   82.1 &
%   37.2 \\
%  &
%   Mistral\textsubscript{7B-Inst} &
%   94.7 &
%   97.2 &
%   97.4 &
%   98.8 &
%   94.7 &
%   91.4 &
%   97.9 &
%   92.8 &
%   92.9 &
%   95.3 &
%   7.3\\
%  &
%   Llama2\textsubscript{13B-Chat} &
%   92.7 &
%   \textbf{100.0} &
%   96.7 &
%   89.7 &
%   91.0 &
%   91.0 &
%   92.5 &
%   89.6 &
%   83.7 &
%   91.8 &
%   16.3 \\
%  &
%   Mixtral\textsubscript{8x7B-Inst} &
%   97.4 &
%   98.0 &
%   99.2 &
%   98.2 &
%   93.7 &
%   98.3 &
%   93.9 &
%   \textbf{98.9} &
%   92.4 &
%   96.3 &
%   6.9 \\
% \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
%   GPT-3.5\textsubscript{turbo} &
%   95.0 &
%   96.0 &
%   99.6 &
%   97.6 &
%   94.2 &
%   \textbf{99.0} &
%   98.0 &
%   93.2 &
%   94.4 &
%   96.4 &
%   \textbf{6.4} \\
%  &
%   GPT-4\textsubscript{turbo} &
%   97.3 &
%   97.2 &
%   98.8 &
%   96.3 &
%   \textbf{99.3} &
%   98.0 &
%   100.0 &
%   93.2 &
%   92.1 &
%   97.0 &
%   7.9 \\
%  &
%   Claude2.1 &
%   \textbf{99.3} &
%   93.3 &
%   \textbf{100.0} &
%   \textbf{100.0} &
%   97.9 &
%   97.6 &
%   \textbf{99.2} &
%   92.3 &
%   \textbf{98.6} &
%   \textbf{97.8} &
%   7.7 \\
% \midrule
% \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
%   92.7 &
%   91.6 &
%   96.5 &
%   93.1 &
%   89.9 &
%   89.5 &
%   92.5 &
%   90.6 &
%   90.2 &
%   85.7 &
%   \\                         
% \bottomrule
% \end{tabular}
% \caption{Faithfulness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% \label{tab:faith_score_table_total}
% \end{center}
% \end{table*}

% \begin{table*}[!h]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{
%     cccccccccccccc}
% \toprule
% \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-12}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{\makecell{Med \\ lit}} & 
% \textbf{Sci-fi} & 
% \textbf{\makecell{Daliy \\ Life}} & 
% \textbf{Booking} & 
% \textbf{\makecell{Booking \\ (RED)}} &
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}}  &
%   BART\textsubscript{large} &
%   49.8 &
%   86.0 &
%   17.0 &
%   23.8 &
%   8.0 &
%   40.1 &
%   55.4 &
%   32.8 &
%   30.8 &
%   31.0 &
%   37.5 &
%   78.0 \\
%  &
%   Flan-T5\textsubscript{large} &
%   43.2 &
%   43.7 &
%   21.2 &
%   19.2 &
%   8.4 &
%   46.5 &
%   42.5 &
%   30.0 &
%   31.1 &
%   33.4 &
%   31.9 &
%   \textbf{38.1} \\
% \midrule
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   63.9 &
%   49.2 &
%   19.5 &
%   18.2 &
%   13.0 &
%   46.4 &
%   27.4 &
%   18.0 &
%   27.8 &
%   23.4 &
%   30.7 &
%   50.9 \\
%  &
%   Mistral\textsubscript{7B-Inst} &
%   \textbf{71.9} &
%   83.5 &
%   46.8 &
%   44.9 &
%   \textbf{37.6} &
%   63.3 &
%   69.1 &
%   55.2 &
%   55.0 &
%   63.8 &
%   59.1 &
%   45.9\\
%  &
%   Llama2\textsubscript{13B-chat} &
%   50.7 &
%   72.6 &
%   27.9 &
%   48.8 &
%   10.8 &
%   37.6 &
%   43.0 &
%   29.7 &
%   37.7 &
%   33.9 &
%   39.3 &
%   61.8 \\
%  &
%   Mixtral\textsubscript{8x7B-Inst} &
%   69.4 &
%   \textbf{92.4} &
%   \textbf{47.8} &
%   50.7 &
%   34.2 &
%   64.1 &
%   72.7 &
%   58.3 &
%   58.3 &
%   62.7 &
%   61.1 &
%   58.2 \\
% \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
%   GPT-3.5\textsubscript{turbo} &
%   53.1 &
%   90.4 &
%   45.1 &
%   \textbf{53.0} &
%   29.0 &
%   66.0 &
%   59.6 &
%   36.4 &
%   47.3 &
%   51.3 &
%   53.1 &
%   61.3 \\
%  &
%   GPT-4\textsubscript{turbo} &
%   66.2 &
%   \textbf{92.4} &
%   47.6 &
%   50.9 &
%   36.6 &
%   \textbf{76.4} &
%   \textbf{76.2} &
%   \textbf{59.8} &
%   \textbf{61.5} &
%   \textbf{67.4} &
%   \textbf{63.5} &
%   55.8 \\
%  &
%   Claude2.1 &
%   53.4 &
%   75.0 &
%   26.4 &
%   36.1 &
%   33.4 &
%   67.5 &
%   53.4 &
%   48.2 &
%   45.0 &
%   44.7 &
%   48.3 &
%   48.6 \\
% \midrule
% \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
%   57.9 &
%   76.1 &
%   33.3 &
%   38.4 &
%   23.4 &
%   56.4 &
%   55.5 &
%   40.9 &
%   43.8 &
%   45.7 & \\
% \bottomrule
% \end{tabular}
% \caption{Completeness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% \label{tab:comp_score_table_total}
% \end{center}
% \end{table*}


% \begin{table*}[!h]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{
%     ccccccccccccccc}
% \toprule
% \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-12}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{\makecell{Med \\ lit}} & 
% \textbf{Sci-fi} & 
% \textbf{\makecell{Daliy \\ Life}} & 
% \textbf{Booking} & 
% \textbf{\makecell{Booking \\ (RED)}} &
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}} &
%   BART\textsubscript{large} &
%   \textbf{90.9} &
%   82.3 &
%   73.3 &
%   81.3 &
%   25.8 &
%   75.7 &
%   83.4 &
%   \textbf{75.3} &
%   68.5 &
%   75.9 &
%   73.2 &
%   65.1 \\
%  &
%   Flan-T5\textsubscript{large} &
%   89.7 &
%   78.0 &
%   \textbf{88.3} &
%   83.3 &
%   35.3 &
%   80.3 &
%   72.3 &
%   59.8 &
%   74.2 &
%   60.6 &
%   72.2 &
%   54.3 \\
% \midrule
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   73.8 &
%   68.3 &
%   40.1 &
%   63.4 &
%   27.3 &
%   75.4 &
%   46.3 &
%   31.7 &
%   46.0 &
%   53.0 &
%   52.5 &
%   48.1 \\
%  &
%   Mistral\textsubscript{7B-Inst}&
%   83.6 &
%   95.0 &
%   78.7 &
%   72.8 &
%   59.8 &
%   78.5 &
%   80.7 &
%   68.7 &
%   75.1 &
%   75.0 &
%   76.8 &
%   35.2 \\
%  &
%   Llama2\textsubscript{13B-chat} &
%   90.5 &
%   94.7 &
%   65.7 &
%   85.6 &
%   39.4 &
%   88.2 &
%   71.6 &
%   57.3 &
%   76.8 &
%   69.4 &
%   73.9 &
%   55.3 \\
%  &
%   Mixtral\textsubscript{8x7B-Inst} &
%   82.8 &
%   92.5 &
%   70.7 &
%   70.2 &
%   49.8 &
%   84.2 &
%   70.0 &
%   69.7 &
%   79.5 &
%   68.4 &
%   73.8 &
%   42.7\\
% \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
% GPT-3.5\textsubscript{turbo} &
%   84.9 &
%   98.0 &
%   87.8 &
%   \textbf{91.4} &
%   65.1 &
%   \textbf{94.1} &
%   72.4 &
%   46.0 &
%   79.7 &
%   78.7 &
%   79.8 &
%   52.0 \\
%  &
%   GPT-4\textsubscript{turbo} &
%   85.8 &
%   \textbf{95.2} &
%   87.8 &
%   90.0 &
%   \textbf{70.1} &
%   87.7 &
%   \textbf{86.1} &
%   \textbf{75.3} &
%   84.5 &
%   79.3 &
%   \textbf{84.2} &
%   \textbf{25.1} \\
%  &
%   Claude2.1 &
%   85.2 &
%   84.0 &
%   76.9 &
%   85.4 &
%   61.7 &
%   83.1 &
%   68.9 &
%   60.7 &
%   \textbf{85.2} &
%   \textbf{86.5} &
%   77.8 &
%   25.8 \\              
% \midrule
% \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
%   85.3 &
%   87.5 &
%   74.4 &
%   80.4 &
%   48.3 &
%   83.0 &
%   72.4 &
%   60.5 &
%   74.4 &
%   71.9 &
% \\
% \bottomrule
% \end{tabular}
% \caption{Conciseness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% \label{tab:conc_score_table_total}
% \end{center}
% \end{table*}


% \begin{table*}[!h]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{
%     cccccccccccccc}
% \toprule
% \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-12}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{\makecell{Med \\ lit}} & 
% \textbf{Sci-fi} & 
% \textbf{\makecell{Daliy \\ Life}} & 
% \textbf{Booking} & 
% \textbf{\makecell{Booking \\ (RED)}} &
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}}  &
%   BART\textsubscript{large} &
%   77.4 &
%   84.0 &
%   60.5 &
%   65.6 &
%   39.8 &
%   65.4 &
%   73.9 &
%   62.4 &
%   60.1 &
%   60.5 &
%   65.0 &
%   44.2 \\
%  &
%   Flan-T5\textsubscript{large} &
%   72.5 &
%   72.6 &
%   65.0 &
%   64.2 &
%   39.5 &
%   64.3 &
%   64.5 &
%   55.2 &
%   64.9 &
%   51.8 &
%   61.4 &
%   33.1 \\
% \midrule
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   73.1 &
%   60.1 &
%   53.2 &
%   52.5 &
%   39.3 &
%   68.5 &
%   54.6 &
%   45.5 &
%   51.6 &
%   52.6 &
%   55.1 &
%   33.9 \\
%  &
%   Mistral\textsubscript{7B-Inst} &
%  \textbf{83.4} &
%   91.9 &
%   74.3 &
%   72.2 &
%   64.0 &
%   77.8 &
%   82.6 &
%   73.2 &
%   74.3 &
%   77.3 &
%   77.1 &
%   27.9 \\
%  &
%   Llama2\textsubscript{13B-chat} &
%   78.0 &
%   89.1 &
%   63.4 &
%   74.7 &
%   47.0 &
%   72.3 &
%   69.0 &
%   59.4 &
%   68.1 &
%   62.4 &
%   68.3 &
%   42.0 \\
%  &
%   Mixtral\textsubscript{8x7B-Inst} &
%  83.2 &
%   94.3 &
%   72.6 &
%   73.0 &
%   59.2 &
%   82.2 &
%   78.9 &
%   73.5 &
%   78.9 &
%   74.5 &
%   77.0 &
%   35.1 \\
% \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
%   GPT-3.5\textsubscript{turbo} &
%   77.7 &
%   94.8 &
%   77.5 &
%   \textbf{80.7} &
%   53.1 &
%   64.4 &
%   56.8 &
%   47.7 &
%   57.7 &
%   57.7 &
%   66.8 &
%   47.1 \\
%  &
%   GPT-4\textsubscript{turbo} &
%   83.1 &
%   \textbf{94.9} &
%   \textbf{78.1} &
%   79.0 &
%   \textbf{68.7} &
%   \textbf{87.4} &
%   \textbf{87.5} &
%   \textbf{77.7} &
%   \textbf{79.7} &
%   \textbf{79.6} &
%   \textbf{81.6} &
%   26.2 \\
%  &
%   Claude2.1 &
%   79.3 &
%   84.1 &
%   67.8 &
%   73.8 &
%   64.3 &
%   82.7 &
%   73.8 &
%   69.6 &
%   74.2 &
%   76.6 &
%   74.6 &
%   \textbf{19.8} \\
% \midrule
% \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
%   78.6 &
%   85.1 &
%   68.0 &
%   70.6 &
%   53.6 &
%   75.9 &
%   73.3 &
%   64.2 &
%   69.3 &
%   67.5 & \\
% \bottomrule
% \end{tabular}
% \caption{Composite score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% \label{tab:cpos_score_table_total}
% \end{center}
% \end{table*}




% % \begin{table*}[!h]
% % \begin{center}
% % \footnotesize
% % \setlength{\tabcolsep}{2.5pt}
% % \renewcommand{\arraystretch}{1.25}
% % \begin{tabular}{
% %     cccccccccccccc}
% % \toprule
% % \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% % \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% % \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% % \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% % \multirow{3}{*}{\makecell{\textbf{DoS}}} \\  
% % \cmidrule(lr){3-7}
% % \cmidrule(lr){8-12}
% % & & 
% % \textbf{News} & 
% % \textbf{Lifestyle} & 
% % \textbf{Report} & 
% % \textbf{\makecell{Med \\ lit}} & 
% % \textbf{Sci-fi} & 
% % \textbf{\makecell{Daliy \\ Life}} & 
% % \textbf{Booking} & 
% % \textbf{\makecell{Booking \\ (RED)}} &
% % \textbf{Interview} & 
% % \textbf{Meeting} & 
% % \\ 
% % \midrule

% % \multirow{2}{*}{\makecell{Non \\ LLM}} &
% %   BART\textsubscript{large} &
% %   91.5 &
% %   83.7 &
% %   91.0 &
% %   91.9 &
% %   85.7 &
% %   80.3 &
% %   82.8 &
% %   79.0 &
% %   81.1 &
% %   74.7 &
% %   84.2 &
% %   17.2 \\
% %  &
% %   Flan-T5\textsubscript{large} &
% %   84.7 &
% %   96.0 &
% %   85.3 &
% %   90.0 &
% %   74.7 &
% %   66.0 &
% %   78.6 &
% %   75.7 &
% %   89.5 &
% %   61.4 &
% %   80.2 &
% %   34.6 \\
% % \midrule
% % \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
% %   Phi-2 &
% %   81.8 &
% %   62.8 &
% %   \textbf{100.0} &
% %   75.8 &
% %   77.6 &
% %   83.6 &
% %   90.0 &
% %   86.9 &
% %   81.1 &
% %   81.3 &
% %   82.1 &
% %   37.2 \\
% %  &
% %   Mistral\textsubscript{7B-Inst} &
% %   94.7 &
% %   97.2 &
% %   97.4 &
% %   98.8 &
% %   94.7 &
% %   91.4 &
% %   97.9 &
% %   95.7 &
% %   92.8 &
% %   92.9 &
% %   95.3 &
% %   7.3\\
% %  &
% %   Llama2\textsubscript{13B-Chat} &
% %   92.7 &
% %   \textbf{100.0} &
% %   96.7 &
% %   89.7 &
% %   91.0 &
% %   91.0 &
% %   92.5 &
% %   91.1 &
% %   89.6 &
% %   83.7 &
% %   91.8 &
% %   16.3 \\
% %  &
% %   Mixtral\textsubscript{8x7B-Inst} &
% %   97.4 &
% %   98.0 &
% %   99.2 &
% %   98.2 &
% %   93.7 &
% %   98.3 &
% %   93.9 &
% %   92.6 &
% %   \textbf{98.9} &
% %   92.4 &
% %   96.3 &
% %   6.9 \\
% % \midrule
% % \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
% %   GPT-3.5\textsubscript{turbo} &
% %   95.0 &
% %   96.0 &
% %   99.6 &
% %   97.6 &
% %   94.2 &
% %   \textbf{99.0} &
% %   98.0 &
% %   \textbf{97.0} &
% %   93.2 &
% %   94.4 &
% %   96.4 &
% %   \textbf{6.4} \\
% %  &
% %   GPT-4\textsubscript{turbo} &
% %   97.3 &
% %   97.2 &
% %   98.8 &
% %   96.3 &
% %   \textbf{99.3} &
% %   98.0 &
% %   100.0 &
% %   98.0 &
% %   93.2 &
% %   92.1 &
% %   97.0 &
% %   7.9 \\
% %  &
% %   Claude2.1 &
% %   \textbf{99.3} &
% %   93.3 &
% %   \textbf{100.0} &
% %   \textbf{100.0} &
% %   97.9 &
% %   97.6 &
% %   \textbf{99.2} &
% %   100.0 &
% %   92.3 &
% %   \textbf{98.6} &
% %   \textbf{97.8} &
% %   7.7 \\
% % \midrule
% % \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
% %   92.7 &
% %   91.6 &
% %   96.5 &
% %   93.1 &
% %   89.9 &
% %   89.5 &
% %   92.5 &
% %   90.6 &
% %   90.2 &
% %   85.7 &
% %   \\                         
% % \bottomrule
% % \end{tabular}
% % \caption{Faithfulness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% % \label{tab:faith_score_table_total}
% % \end{center}
% % \end{table*}

% % \begin{table*}[!h]
% % \begin{center}
% % \footnotesize
% % \setlength{\tabcolsep}{2.5pt}
% % \renewcommand{\arraystretch}{1.25}
% % \begin{tabular}{
% %     cccccccccccccc}
% % \toprule
% % \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% % \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% % \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% % \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% % \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% % \cmidrule(lr){3-7}
% % \cmidrule(lr){8-12}
% % & & 
% % \textbf{News} & 
% % \textbf{Lifestyle} & 
% % \textbf{Report} & 
% % \textbf{\makecell{Med \\ lit}} & 
% % \textbf{Sci-fi} & 
% % \textbf{\makecell{Daliy \\ Life}} & 
% % \textbf{Booking} & 
% % \textbf{\makecell{Booking \\ (RED)}} &
% % \textbf{Interview} & 
% % \textbf{Meeting} & 
% % \\ 
% % \midrule

% % \multirow{2}{*}{\makecell{Non \\ LLM}}  &
% %   BART\textsubscript{large} &
% %   49.8 &
% %   86.0 &
% %   17.0 &
% %   23.8 &
% %   8.0 &
% %   40.1 &
% %   55.4 &
% %   32.8 &
% %   30.8 &
% %   31.0 &
% %   37.5 &
% %   78.0 \\
% %  &
% %   Flan-T5\textsubscript{large} &
% %   43.2 &
% %   43.7 &
% %   21.2 &
% %   19.2 &
% %   8.4 &
% %   46.5 &
% %   42.5 &
% %   30.0 &
% %   31.1 &
% %   33.4 &
% %   31.9 &
% %   \textbf{38.1} \\
% % \midrule
% % \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
% %   Phi-2 &
% %   63.9 &
% %   49.2 &
% %   19.5 &
% %   18.2 &
% %   13.0 &
% %   46.4 &
% %   27.4 &
% %   18.0 &
% %   27.8 &
% %   23.4 &
% %   30.7 &
% %   50.9 \\
% %  &
% %   Mistral\textsubscript{7B-Inst} &
% %   \textbf{71.9} &
% %   83.5 &
% %   46.8 &
% %   44.9 &
% %   \textbf{37.6} &
% %   63.3 &
% %   69.1 &
% %   55.2 &
% %   55.0 &
% %   63.8 &
% %   59.1 &
% %   45.9\\
% %  &
% %   Llama2\textsubscript{13B-chat} &
% %   50.7 &
% %   72.6 &
% %   27.9 &
% %   48.8 &
% %   10.8 &
% %   37.6 &
% %   43.0 &
% %   29.7 &
% %   37.7 &
% %   33.9 &
% %   39.3 &
% %   61.8 \\
% %  &
% %   Mixtral\textsubscript{8x7B-Inst} &
% %   69.4 &
% %   \textbf{92.4} &
% %   \textbf{47.8} &
% %   50.7 &
% %   34.2 &
% %   64.1 &
% %   72.7 &
% %   58.3 &
% %   58.3 &
% %   62.7 &
% %   61.1 &
% %   58.2 \\
% % \midrule
% % \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
% %   GPT-3.5\textsubscript{turbo} &
% %   53.1 &
% %   90.4 &
% %   45.1 &
% %   \textbf{53.0} &
% %   29.0 &
% %   66.0 &
% %   59.6 &
% %   36.4 &
% %   47.3 &
% %   51.3 &
% %   53.1 &
% %   61.3 \\
% %  &
% %   GPT-4\textsubscript{turbo} &
% %   66.2 &
% %   \textbf{92.4} &
% %   47.6 &
% %   50.9 &
% %   36.6 &
% %   \textbf{76.4} &
% %   \textbf{76.2} &
% %   \textbf{59.8} &
% %   \textbf{61.5} &
% %   \textbf{67.4} &
% %   \textbf{63.5} &
% %   55.8 \\
% %  &
% %   Claude2.1 &
% %   53.4 &
% %   75.0 &
% %   26.4 &
% %   36.1 &
% %   33.4 &
% %   67.5 &
% %   53.4 &
% %   48.2 &
% %   45.0 &
% %   44.7 &
% %   48.3 &
% %   48.6 \\
% % \midrule
% % \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
% %   57.9 &
% %   76.1 &
% %   33.3 &
% %   38.4 &
% %   23.4 &
% %   56.4 &
% %   55.5 &
% %   40.9 &
% %   43.8 &
% %   45.7 & \\
% % \bottomrule
% % \end{tabular}
% % \caption{Completeness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% % \label{tab:comp_score_table_total}
% % \end{center}
% % \end{table*}


% % \begin{table*}[!h]
% % \begin{center}
% % \footnotesize
% % \setlength{\tabcolsep}{2.5pt}
% % \renewcommand{\arraystretch}{1.25}
% % \begin{tabular}{
% %     ccccccccccccccc}
% % \toprule
% % \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% % \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% % \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% % \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% % \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% % \cmidrule(lr){3-7}
% % \cmidrule(lr){8-12}
% % & & 
% % \textbf{News} & 
% % \textbf{Lifestyle} & 
% % \textbf{Report} & 
% % \textbf{\makecell{Med \\ lit}} & 
% % \textbf{Sci-fi} & 
% % \textbf{\makecell{Daliy \\ Life}} & 
% % \textbf{Booking} & 
% % \textbf{\makecell{Booking \\ (RED)}} &
% % \textbf{Interview} & 
% % \textbf{Meeting} & 
% % \\ 
% % \midrule

% % \multirow{2}{*}{\makecell{Non \\ LLM}} &
% %   BART\textsubscript{large} &
% %   \textbf{90.9} &
% %   82.3 &
% %   73.3 &
% %   81.3 &
% %   25.8 &
% %   75.7 &
% %   83.4 &
% %   \textbf{75.3} &
% %   68.5 &
% %   75.9 &
% %   73.2 &
% %   65.1 \\
% %  &
% %   Flan-T5\textsubscript{large} &
% %   89.7 &
% %   78.0 &
% %   \textbf{88.3} &
% %   83.3 &
% %   35.3 &
% %   80.3 &
% %   72.3 &
% %   59.8 &
% %   74.2 &
% %   60.6 &
% %   72.2 &
% %   54.3 \\
% % \midrule
% % \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
% %   Phi-2 &
% %   73.8 &
% %   68.3 &
% %   40.1 &
% %   63.4 &
% %   27.3 &
% %   75.4 &
% %   46.3 &
% %   31.7 &
% %   46.0 &
% %   53.0 &
% %   52.5 &
% %   48.1 \\
% %  &
% %   Mistral\textsubscript{7B-Inst}&
% %   83.6 &
% %   95.0 &
% %   78.7 &
% %   72.8 &
% %   59.8 &
% %   78.5 &
% %   80.7 &
% %   68.7 &
% %   75.1 &
% %   75.0 &
% %   76.8 &
% %   35.2 \\
% %  &
% %   Llama2\textsubscript{13B-chat} &
% %   90.5 &
% %   94.7 &
% %   65.7 &
% %   85.6 &
% %   39.4 &
% %   88.2 &
% %   71.6 &
% %   57.3 &
% %   76.8 &
% %   69.4 &
% %   73.9 &
% %   55.3 \\
% %  &
% %   Mixtral\textsubscript{8x7B-Inst} &
% %   82.8 &
% %   92.5 &
% %   70.7 &
% %   70.2 &
% %   49.8 &
% %   84.2 &
% %   70.0 &
% %   69.7 &
% %   79.5 &
% %   68.4 &
% %   73.8 &
% %   42.7\\
% % \midrule
% % \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
% % GPT-3.5\textsubscript{turbo} &
% %   84.9 &
% %   98.0 &
% %   87.8 &
% %   \textbf{91.4} &
% %   65.1 &
% %   \textbf{94.1} &
% %   72.4 &
% %   46.0 &
% %   79.7 &
% %   78.7 &
% %   79.8 &
% %   52.0 \\
% %  &
% %   GPT-4\textsubscript{turbo} &
% %   85.8 &
% %   \textbf{95.2} &
% %   87.8 &
% %   90.0 &
% %   \textbf{70.1} &
% %   87.7 &
% %   \textbf{86.1} &
% %   \textbf{75.3} &
% %   84.5 &
% %   79.3 &
% %   \textbf{84.2} &
% %   \textbf{25.1} \\
% %  &
% %   Claude2.1 &
% %   85.2 &
% %   84.0 &
% %   76.9 &
% %   85.4 &
% %   61.7 &
% %   83.1 &
% %   68.9 &
% %   60.7 &
% %   \textbf{85.2} &
% %   \textbf{86.5} &
% %   77.8 &
% %   25.8 \\              
% % \midrule
% % \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
% %   85.3 &
% %   87.5 &
% %   74.4 &
% %   80.4 &
% %   48.3 &
% %   83.0 &
% %   72.4 &
% %   60.5 &
% %   74.4 &
% %   71.9 &
% % \\
% % \bottomrule
% % \end{tabular}
% % \caption{Conciseness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% % \label{tab:conc_score_table_total}
% % \end{center}
% % \end{table*}


% % \begin{table*}[!h]
% % \begin{center}
% % \footnotesize
% % \setlength{\tabcolsep}{2.5pt}
% % \renewcommand{\arraystretch}{1.25}
% % \begin{tabular}{
% %     cccccccccccccc}
% % \toprule
% % \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% % \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% % \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
% % \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} &
% % \multirow{3}{*}{\makecell{\textbf{DoS}}} \\ 
% % \cmidrule(lr){3-7}
% % \cmidrule(lr){8-12}
% % & & 
% % \textbf{News} & 
% % \textbf{Lifestyle} & 
% % \textbf{Report} & 
% % \textbf{\makecell{Med \\ lit}} & 
% % \textbf{Sci-fi} & 
% % \textbf{\makecell{Daliy \\ Life}} & 
% % \textbf{Booking} & 
% % \textbf{\makecell{Booking \\ (RED)}} &
% % \textbf{Interview} & 
% % \textbf{Meeting} & 
% % \\ 
% % \midrule

% % \multirow{2}{*}{\makecell{Non \\ LLM}}  &
% %   BART\textsubscript{large} &
% %   77.4 &
% %   84.0 &
% %   60.5 &
% %   65.6 &
% %   39.8 &
% %   65.4 &
% %   73.9 &
% %   62.4 &
% %   60.1 &
% %   60.5 &
% %   65.0 &
% %   44.2 \\
% %  &
% %   Flan-T5\textsubscript{large} &
% %   72.5 &
% %   72.6 &
% %   65.0 &
% %   64.2 &
% %   39.5 &
% %   64.3 &
% %   64.5 &
% %   55.2 &
% %   64.9 &
% %   51.8 &
% %   61.4 &
% %   33.1 \\
% % \midrule
% % \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
% %   Phi-2 &
% %   73.1 &
% %   60.1 &
% %   53.2 &
% %   52.5 &
% %   39.3 &
% %   68.5 &
% %   54.6 &
% %   45.5 &
% %   51.6 &
% %   52.6 &
% %   55.1 &
% %   33.9 \\
% %  &
% %   Mistral\textsubscript{7B-Inst} &
% %  \textbf{83.4} &
% %   91.9 &
% %   74.3 &
% %   72.2 &
% %   64.0 &
% %   77.8 &
% %   82.6 &
% %   73.2 &
% %   74.3 &
% %   77.3 &
% %   77.1 &
% %   27.9 \\
% %  &
% %   Llama2\textsubscript{13B-chat} &
% %   78.0 &
% %   89.1 &
% %   63.4 &
% %   74.7 &
% %   47.0 &
% %   72.3 &
% %   69.0 &
% %   59.4 &
% %   68.1 &
% %   62.4 &
% %   68.3 &
% %   42.0 \\
% %  &
% %   Mixtral\textsubscript{8x7B-Inst} &
% %  83.2 &
% %   94.3 &
% %   72.6 &
% %   73.0 &
% %   59.2 &
% %   82.2 &
% %   78.9 &
% %   73.5 &
% %   78.9 &
% %   74.5 &
% %   77.0 &
% %   35.1 \\
% % \midrule
% % \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
% %   GPT-3.5\textsubscript{turbo} &
% %   77.7 &
% %   94.8 &
% %   77.5 &
% %   \textbf{80.7} &
% %   53.1 &
% %   64.4 &
% %   56.8 &
% %   47.7 &
% %   57.7 &
% %   57.7 &
% %   66.8 &
% %   47.1 \\
% %  &
% %   GPT-4\textsubscript{turbo} &
% %   83.1 &
% %   \textbf{94.9} &
% %   \textbf{78.1} &
% %   79.0 &
% %   \textbf{68.7} &
% %   \textbf{87.4} &
% %   \textbf{87.5} &
% %   \textbf{77.7} &
% %   \textbf{79.7} &
% %   \textbf{79.6} &
% %   \textbf{81.6} &
% %   26.2 \\
% %  &
% %   Claude2.1 &
% %   79.3 &
% %   84.1 &
% %   67.8 &
% %   73.8 &
% %   64.3 &
% %   82.7 &
% %   73.8 &
% %   69.6 &
% %   74.2 &
% %   76.6 &
% %   74.6 &
% %   \textbf{19.8} \\
% % \midrule
% % \multicolumn{2}{c}{\textbf{Avg. Score in Domain}} &
% %   78.6 &
% %   85.1 &
% %   68.0 &
% %   70.6 &
% %   53.6 &
% %   75.9 &
% %   73.3 &
% %   64.2 &
% %   69.3 &
% %   67.5 & \\
% % \bottomrule
% % \end{tabular}
% % \caption{Composite score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain. The bottom row represents the average score for each domain.}
% % \label{tab:cpos_score_table_total}
% % \end{center}
% % \end{table*}



==> tables/model_error_type_total.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{16pt}
\begin{center}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{\textbf{LLM Type}} & \multirow{2}{*}{\textbf{Summ. Model}} & \multicolumn{3}{c}{\textbf{Intrinsic}} & \textbf{Extrinsic} & \multirow{2}{*}{\textbf{Overall}} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-6}
                                    &                                      & \textbf{EntE} & \textbf{RelE} & \textbf{SenE} & \textbf{OutE} &                                      \\ \midrule
\multirow{2}{*}{Non-LLM} & BART                                 & 4.33\%        & 1.84\%        & 3.81\%        & 5.38\%        & 15.35\%                             \\
                                    & FLAN-T5                              & 4.13\%        & 1.28\%        & 7.82\%        & 10.95\%       & 24.18\%                             \\                               
                                    \midrule
\multirow{4}{*}{\makecell{Open \\ Source \\ LLM}}    
& Phi-2                                & 2.31\%        & 2.02\%        & 4.90\%        & 8.93\%        & 18.16\%                             \\ 
& Mistral 7B                           & 0.92\%        & 0.25\%        & 0.42\%        & 2.77\%        & 4.36\%                              \\
& Llama2 13B                           & 0.74\%        & 1.29\%        & 2.02\%        & 5.33\%        & 9.38\%                              \\
& Mixtral 8x7B                         & 0.41\%        & 0.41\%        & 0.62\%        & 1.10\%        & 2.55\%                              \\ \midrule
\multirow{3}{*}{\makecell{Prop. \\ LLM}}     
                                    & GPT-3.5 turbo                        & 0.11\%        & 0.21\%        & 0.53\%        & 2.43\%        & 3.28\%                              \\
                                    & GPT-4 turbo                          & 0.10\%        & 0.51\%        & 0.51\%        & 2.13\%        & 3.24\%                              \\
                                    & Claude2.1                            & 0.36\%        & 0.12\%        & 0.12\%        & 1.31\%        & 1.91\%                              \\ \midrule
                                    & All models                           & 1.28\%        & 0.75\%        & 1.90\%        & 3.86\%        & 7.79\%                              \\ 
\bottomrule
\end{tabular}
\caption{Percentage of sentence-level factual errors across the nine models in \algname, with errors categorized based on majority agreement among annotators. -> \tobefilled}
\label{tab:Proportion_error}
\end{center}
\end{table*}

==> tables/source_data_half.tex <==
% User
% \begin{table}[t]
% \begin{center}
% \footnotesize
% \renewcommand{\arraystretch}{2}
% \setlength{\tabcolsep}{1.5pt}
% \begin{tabular}{|c|c|c|c|}
% \Xhline{3\arrayrulewidth}
% \textbf{Type} & \textbf{Length} & \textbf{Domain} & \textbf{Dataset} \\
% \Xhline{3\arrayrulewidth}
% \multirow{5}{*}{\makecell{Non- \\ dialogue}} & \multirow{2}{*}{Short} & \makecell{News \\ Article}& \makecell{CNNDM \\ \cite{nallapati-etal-2016-abstractive}} \\
% \cline{3-4}
%  & & Lifestyle & \makecell{WikiHow \\ \cite{koupaee2018wikihow}} \\
% \cline{2-4}
%  & \multirow{3}{*}{Long} & Report & \makecell{GovReport \\ \cite{huang-etal-2021-efficient}} \\
% \cline{3-4}
%  & & \makecell{Medical \\ Literature} & \makecell{Pubmed \\ \cite{cohan-etal-2018-discourse}} \\
% \cline{3-4}
%  & & Sci-fiction & \makecell{SQuALITY \\ \cite{wang-etal-2022-squality}} \\
% \hline
% \multirow{4}{*}{Dialogue} & \multirow{2}{*}{Short} & Daily Life & \makecell{DialogSum \\ \cite{chen-etal-2021-dialogsum}} \\
% \cline{3-4}
%  & & Booking & \makecell{MultiWOZ \\ \cite{budzianowski-etal-2018-multiwoz}} \\
% \cline{2-4}
%  & \multirow{2}{*}{Long} & Interview & \makecell{MediaSum \\ \cite{zhu-etal-2021-mediasum}} \\
% \cline{3-4}
%  & & Meeting & \makecell{MeetingBank \\ \cite{hu-etal-2023-meetingbank}} \\
% \Xhline{3\arrayrulewidth}
% \end{tabular}
% \caption{Source datasets used in \algname{}. Detailed descriptions and statistics of the source datasets is in Appendix.}
% \label{table:datasets}
% \end{center}
% \end{table}

% \begin{table}[t]
% \begin{center}
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{c c l} 
% \toprule
% \multicolumn{1}{c}{\textbf{Length}} & \multicolumn{1}{c}{\textbf{Domain}} & \multicolumn{1}{c}{\textbf{Dataset}} \\  
% \midrule
% \multicolumn{3}{c}{Non-dialogue} \\
% \midrule
% Short & News & CNNDM \cite{nallapati-etal-2016-abstractive} \\
% Short & Lifestyle & WikiHow \cite{koupaee2018wikihow} \\
% Long & Report & GovReport \cite{huang-etal-2021-efficient} \\
% Long & Med lit & Pubmed \cite{cohan-etal-2018-discourse} \\
% Long & Sci-fiction & SQuALITY \cite{wang-etal-2022-squality} \\
% \midrule
% \multicolumn{3}{c}{Dialogue} \\
% \midrule
% Short & Daily life & DialogSum \cite{chen-etal-2021-dialogsum} \\
% Short & Booking & MultiWOZ \cite{budzianowski-etal-2018-multiwoz} \\
% Short & \makecell{Booking\\(redacted)} & MultiWOZ\_RED \\
% Long & Interview & MediaSum \cite{zhu-etal-2021-mediasum} \\
% Long & Meeting & MeetingBank \cite{hu-etal-2023-meetingbank} \\
% \bottomrule
% \end{tabular}
% \caption{Source datasets used in \algname{}. Detailed descriptions and statistics of the source datasets are in the Appendix.}
% \label{table:datasets}
% \end{center}
% \end{table}

==> tables/sum_model_score_table_total.tex <==
\begin{table*}[t]
\begin{center}
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{15pt}
\begin{tabular}{cccccc}
\Xhline{3\arrayrulewidth}
\textbf{Type} & \textbf{Summ. Model} & \textbf{Faithfulness} & \textbf{Completeness} & \textbf{Conciseness} & \textbf{Avg. Score} \\ 
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\makecell{Non \\ LLM}} 
& BART-large        & 84.7          & 39.1          & 70.1          & 64.6          \\
& Flan-T5-large     & 80.7          & 33.6          & 68.6          & 61.0          \\
\cmidrule(lr){1-6}
\multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} 
& Phi-2             & 80.4          & 32.3          & 49.5          & 54.1          \\
& Mistral-7B-Inst   & 95.2          & 62.5          & 72.0          & 76.6          \\
& Llama2-chat-13B   & 92.7          & 42.7          & 71.4          & 68.9          \\
& Mixtral-8x7B-Inst & 96.8          & 62.6          & 68.9          & 76.1          \\
\cmidrule(lr){1-6}
\multirow{3}{*}{\makecell{Prop. \\ LLM}} 
& GPT-3.5-turbo     & 96.3          & 56.1          & 75.6          & 76.0          \\
& GPT-4             & 96.9          & \textbf{65.2} & \textbf{80.0} & \textbf{80.7} \\
& Claude2.1         & \textbf{97.6} & 51.6          & 74.4          & 74.6  \\     
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Performance of summarization models along three dimensions in CSEVAL. We highlight the best performance for each column.}
\label{tab:summ_model_score}
\end{center}
\end{table*}


==> tables/summarization_model_score/before_editing/comp_score_table.tex <==
\begin{table*}[t]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{
    ccccccccccccc}
\Xhline{3\arrayrulewidth}
\multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
\multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
\multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
\multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} \\ 
\cmidrule(lr){3-7}
\cmidrule(lr){8-12}
& & 
\textbf{News} & 
\textbf{Lifestyle} & 
\textbf{Report} & 
\textbf{\makecell{Med \\ lit}} & 
\textbf{Sci-fi} & 
\textbf{\makecell{Daliy \\ Life}} & 
\textbf{Booking} & 
\textbf{\makecell{Booking \\ (RED)}} &
\textbf{Interview} & 
\textbf{Meeting} & 
\\ 
\midrule

\multirow{2}{*}{\makecell{Non \\ LLM}} &
  BART-large &
  50.0 &
  86.0 &
  17.0 &
  24.6 &
  7.4 &
  38.4 &
  54.9 &
  32.3 &
  31.4 &
  31.0 &
  37.3 \\
 &
  Flan-T5-large &
  44.7 &
  45.0 &
  22.3 &
  19.2 &
  8.4 &
  45.7 &
  44.1 &
  29.6 &
  31.9 &
  33.4 &
  32.4 \\
\midrule
\multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
  Phi-2 &
  64.0 &
  49.2 &
  19.5 &
  18.2 &
  12.9 &
  46.4 &
  28.1 &
  16.5 &
  27.8 &
  23.4 &
  30.6 \\
 &
  Mistral-7B-Inst &
  \textbf{71.9} &
  83.5 &
  46.6 &
  45.2 &
  \textbf{37.5} &
  63.6 &
  71.6 &
  55.2 &
  55.3 &
  64.2 &
  59.4 \\
 &
  Llama2-13B-Chat &
  54.5 &
  72.6 &
  28.3 &
  48.8 &
  10.8 &
  37.6 &
  44.3 &
  29.7 &
  37.7 &
  33.9 &
  39.8 \\
 &
  Mixtral-8x7B-Inst &
  67.6 &
  \textbf{93.4} &
  \textbf{48.0} &
  50.7 &
  34.8 &
  69.8 &
  72.7 &
  57.9 &
  58.6 &
  63.2 &
  61.7 \\
\midrule
\multirow{3}{*}{\makecell{Prop. \\ LLM}} &
  GPT-3.5-turbo &
  54.6 &
  90.4 &
  45.3 &
  \textbf{52.6} &
  29.7 &
  68.7 &
  59.6 &
  35.4 &
  48.4 &
  51.7 &
  53.6 \\
 &
  GPT-4-turbo &
  64.9 &
  92.4 &
  46.6 &
  51.7 &
  36.8 &
  \textbf{76.3} &
  \textbf{78.1} &
  \textbf{59.4} &
  \textbf{60.9} &
  \textbf{67.4} &
  \textbf{63.4} \\
 &
  Claude2.1 &
  55.0 &
  75.0 &
  28.4 &
  39.7 &
  33.8 &
  64.9 &
  56.7 &
  48.6 &
  45.7 &
  44.7 &
  49.2 \\                         
\bottomrule
\end{tabular}
\caption{Completeness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain.}
\end{center}
\end{table*}


==> tables/summarization_model_score/before_editing/conc_score_table.tex <==
\begin{table*}[t]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{
    ccccccccccccc}
\Xhline{3\arrayrulewidth}
\multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
\multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
\multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{5}{c}{\textbf{Dialogue}} & 
\multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} \\ 
\cmidrule(lr){3-7}
\cmidrule(lr){8-12}
& & 
\textbf{News} & 
\textbf{Lifestyle} & 
\textbf{Report} & 
\textbf{\makecell{Med \\ lit}} & 
\textbf{Sci-fi} & 
\textbf{\makecell{Daliy \\ Life}} & 
\textbf{Booking} & 
\textbf{\makecell{Booking \\ (RED)}} &
\textbf{Interview} & 
\textbf{Meeting} & 
\\ 
\midrule

\multirow{2}{*}{\makecell{Non \\ LLM}} &
  BART-large &
  93.9 &
  82.3 &
  74.7 &
  81.3 &
  26.1 &
  73.7 &
  85.7 &
  \textbf{77.7} &
  70.8 &
  77.2 &
  74.3 \\
 &
  Flan-T5-large &
  89.7 &
  78.0 &
  \textbf{88.3} &
  83.3 &
  36.7 &
  79.0 &
  74.6 &
  58.5 &
  76.1 &
  60.6 &
  72.5 \\
\midrule
\multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
  Phi-2 &
  76.1 &
  68.3 &
  40.1 &
  63.4 &
  25.7 &
  77.0 &
  47.3 &
  29.1 &
  46.9 &
  54.0 &
  52.8 \\
 &
  Mistral-7B-Inst &
  83.6 &
  95.0 &
  78.7 &
  72.8 &
  61.1 &
  79.8 &
  82.2 &
  68.7 &
  76.7 &
  76.8 &
  77.5 \\
 &
  Llama2-13B-Chat &
  \textbf{91.4} &
  94.7 &
  67.1 &
  85.6 &
  39.4 &
  88.2 &
  72.5 &
  58.3 &
  76.8 &
  69.4 &
  74.3 \\
 &
  Mixtral-8x7B-Inst &
  81.3 &
  92.5 &
  71.2 &
  70.2 &
  52.0 &
  88.3 &
  70.0 &
  70.4 &
  81.0 &
  71.0 &
  74.8 \\
\midrule
\multirow{3}{*}{\makecell{Prop. \\ LLM}} &
  GPT-3.5-turbo &
  86.9 &
  98.0 &
  87.8 &
  \textbf{91.4} &
  65.1 &
  \textbf{94.1} &
  72.4 &
  46.0 &
  81.2 &
  79.7 &
  80.3 \\
 &
  GPT-4-turbo &
  89.6 &
  \textbf{95.2} &
  87.8 &
  90.8 &
  \textbf{74.2} &
  87.7 &
  \textbf{86.1} &
  75.3 &
  84.2 &
  82.3 &
  \textbf{85.3} \\
 &
  Claude2.1 &
  86.7 &
  84.0 &
  80.6 &
  89.1 &
  64.3 &
  82.1 &
  70.3 &
  62.4 &
  \textbf{85.2} &
  \textbf{86.5} &
  79.1 \\                         
\bottomrule
\end{tabular}
\caption{Conciseness score on \algname{} across ten domains. The best performance is highlighted in \textbf{bold} for each domain.}
\end{center}
\end{table*}


% \begin{table*}[t]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1.25}
% % \begin{tabular}{
% %   >{\centering\arraybackslash}m{0.5cm} 
% %   >{\centering\arraybackslash}m{1.5cm} 
% %   >{\centering\arraybackslash}m{0.6cm} 
% %   >{\centering\arraybackslash}m{0.9cm} 
% %   >{\centering\arraybackslash}m{0.7cm} 
% %   >{\centering\arraybackslash}m{0.7cm} 
% %   >{\centering\arraybackslash}m{0.7cm} 
% %   >{\centering\arraybackslash}m{0.8cm} 
% %   >{\centering\arraybackslash}m{0.8cm} 
% %   >{\centering\arraybackslash}m{1cm} 
% %   >{\centering\arraybackslash}m{1cm} 
% %   >{\centering\arraybackslash}m{1cm}
% % }
% \begin{tabular}{
%     cccccccccccc}
% \Xhline{3\arrayrulewidth}
% \multirow{3}{*}{\makecell{Model \\ Type}} &
% \multirow{3}{*}{\makecell{Summ. \\ Model}} &
% \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} 
% & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{4}{c}{\textbf{Dialogue}} & 
% \multirow{2}{*}{\makecell{Avg. \\ Score}} \\ 
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-11}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{Medical} & 
% \textbf{Sci-fi} & 
% \textbf{Daily Life} & 
% \textbf{Booking} & 
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}} & BART & 0.915 & 0.837 & 0.910 & 0.919 & 0.857 & 0.803 & 0.828 & 0.811 & 0.747 & 0.847 \\
%                          & Flan-T5 & 0.847 & 0.960 & 0.853 & 0.900 & 0.747 & 0.660 & 0.786 & 0.895 & 0.614 & 0.807 \\ 
%                          \midrule

% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} 
%                           & Phi-2 & 0.818 & 0.628 & \textbf{1.000} & 0.758 & 0.776 & 0.836 & 0.900 & 0.811 & 0.813 & 0.815 \\
%                           & Mistral 7B & 0.947 & 0.972 & 0.974 & 0.988 & 0.947 & 0.914 & 0.979 & 0.928 & 0.929 & 0.953 \\
%                           & Llama2 13B & 0.927 & \textbf{1.000} & 0.967 & 0.897 & 0.910 & 0.910 & 0.925 & 0.896 & 0.837 & 0.919 \\
%                           & Mixtral 8x7B & 0.974 & 0.980 & 0.992 & 0.982 & 0.937 & 0.983 & 0.939 & \textbf{0.989} & 0.924 & 0.967 \\ \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} 
%                           & GPT-3.5-turbo & 0.950 & 0.960 & 0.996 & 0.976 & 0.942 & \textbf{0.990} & 0.980 & 0.932 & 0.944 & 0.963 \\
%                           & Claude2.1 & \textbf{0.993} & 0.933 & \textbf{1.000} & \textbf{1.000} & 0.979 & 0.976 & 0.992 & 0.923 & \textbf{0.986} & \textbf{0.976} \\ 
%                           & GPT-4-turbo & 0.973 & 0.972 & 0.988 & 0.963 & \textbf{0.993} & 0.980 & \textbf{1.000} & 0.932 & 0.921 & 0.969 \\
                          
                          
% \Xhline{3\arrayrulewidth}
% \end{tabular}
% \caption{Fatihfulness score on \algname{} across nine domain. the best performance is highlighted in \textbf{bold} for each domain 각각의 score 테이블로 만들고 appendix에 넣고 나중에 필요한 것만 가져오기}
% \label{tab:Faith_score_table}
% \end{center}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
% \footnotesize
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{
%     cccccccccccc}
% \Xhline{3\arrayrulewidth}
% \multirow{3}{*}{\makecell{\textbf{Model} \\ \textbf{Type}}} &
% \multirow{3}{*}{\makecell{\textbf{Summ.} \\ \textbf{Model}}} &
% % \multicolumn{9}{c}{\textbf{Document Type}} \\ \cmidrule(lr){3-11} & & 
% \multicolumn{5}{c}{\textbf{Non-Dialogue}} & \multicolumn{4}{c}{\textbf{Dialogue}} & 
% \multirow{3}{*}{\makecell{\textbf{Avg.} \\ \textbf{Score}}} \\ 
% \cmidrule(lr){3-7}
% \cmidrule(lr){8-11}
% & & 
% \textbf{News} & 
% \textbf{Lifestyle} & 
% \textbf{Report} & 
% \textbf{Med lit} & 
% \textbf{Sci-fi} & 
% \textbf{Daily Life} & 
% \textbf{Booking} & 
% \textbf{Interview} & 
% \textbf{Meeting} & 
% \\ 
% \midrule

% \multirow{2}{*}{\makecell{Non \\ LLM}} &
% BART &
%   86.7 &
%   79.6 &
%   73.7 &
%   76.9 &
%   24.1 &
%   67.3 &
%   77.7 &
%   66.1 &
%   74.2 &
%   69.6 \\
%  &
%   Flan-T5 &
%   84.2 &
%   78.0 &
%   \textbf{87.0} &
%   79.3 &
%   33.3 &
%   74.7 &
%   69.7 &
%   69.9 &
%   59.5 &
%   70.6 \\
% \midrule
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   70.5 &
%   68.3 &
%   40.1 &
%   63.4 &
%   24.2 &
%   71.5 &
%   46.3 &
%   34.8 &
%   52.3 &
%   52.4 \\
%  &
%   Mistral-7B &
%   77.1 &
%   94.0 &
%   75.6 &
%   67.6 &
%   57.8 &
%   69.7 &
%   74.4 &
%   67.4 &
%   73.5 &
%   73.0 \\
%  &
%   Llama2-13B &
%   \textbf{89.9} &
%   91.3 &
%   65.9 &
%   82.3 &
%   34.6 &
%   79.2 &
%   69.2 &
%   75.0 &
%   69.4 &
%   73.0 \\
%  &
%   Mixtral-8x7B &
%   75.9 &
%   89.0 &
%   67.0 &
%   67.8 &
%   51.1 &
%   75.0 &
%   59.9 &
%   71.9 &
%   66.2 &
%   69.3 \\
% \midrule
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
%   GPT-3.5-turbo &
%   83.7 &
%   94.7 &
%   86.0 &
%   \textbf{88.3} &
%   62.1 &
%   \textbf{86.2} &
%   67.1 &
%   72.8 &
%   72.5 &
%   79.3 \\
%  &
%   GPT-4-turbo &
%   83.5 &
%   \textbf{95.2} &
%   86.1 &
%   87.9 &
%   \textbf{68.6} &
%   76.3 &
%   \textbf{82.1} &
%   78.1 &
%   71.5 &
%   \textbf{81.0} \\
%  &
%   Claude2.1 &
%   81.6 &
%   80.3 &
%   78.1 &
%   87.5 &
%   62.9 &
%   71.0 &
%   66.0 &
%   \textbf{81.9} &
%   \textbf{84.0} &
%   77.0 \\   
% \Xhline{3\arrayrulewidth}
% \end{tabular}
% \caption{Conciseness score on \algname{} across nine domains. The best performance is highlighted in \textbf{bold} for each domain. 각각의 score 테이블로 만들고 appendix에 넣고 나중에 필요한 것만 가져오기}
% \label{tab:Faith_score_table}
% \end{center}
% \end{table*}


==> tables/summarization_model_score/before_editing/redaction_analysis.tex <==
\begin{table*}[]
\begin{center}
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{9pt}
\begin{tabular}{cccccccc}
\Xhline{3\arrayrulewidth}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{Faithfulness}} & \multicolumn{2}{c}{\textbf{Completeness}} & \multicolumn{2}{c}{\textbf{Conciseness}} \\ 
\cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8} 
\textbf{Type} & \textbf{Model} & \textbf{Unredact} & \textbf{Redact} & \textbf{Unredact} & \textbf{Redact} & \textbf{Unredact} & \textbf{Redact} \\ \midrule
\multirow{2}{*}{\makecell{Non \\ LLM}}         
                                 & BART        & 82.8        & 79.0 \textcolor{red}{(-3.8)}         & 55.7        & 36.3 \textcolor{red}{(-19.4)}       & 77.7       & 74.3 \textcolor{red}{(-3.4)}       \\
                                 & Flan-T5     & 78.6        & 75.7 \textcolor{red}{(-2.9)}        & 45.2        & 30.5 \textcolor{red}{(-14.7)}       & 69.7       & 50.5 \textcolor{red}{(-19.2)}       \\
                                 \midrule
\multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} & Phi-2             & 90.0        & 86.9 \textcolor{red}{(-3.1)}        & 31.5        & 15.0 \textcolor{red}{(-16.5)}        & 46.3       & 24.5 \textcolor{red}{(-21.9)}       \\
                                 & Mistral-7B   & 97.9        & 95.7 \textcolor{red}{(-2.3)}        & 74.6        & 57.9 \textcolor{red}{(-16.7)}       & 74.4       & 63.3 \textcolor{red}{(-11.1)}       \\
                                 & Llama2 13B   & 92.5        & 91.1 \textcolor{red}{(-1.4)}        & 45.7        & 30.1 \textcolor{red}{(-15.6)}       & 69.2       & 55.0 \textcolor{red}{(-14.2)}        \\
                                 & Mixtral-8x7B & 93.9        & 92.6 \textcolor{red}{(-1.4)}        & 76.1        & 60.7 \textcolor{red}{(-15.4)}       & 59.9       & 62.4 \textcolor[rgb]{0,0.6,0}{(2.5)}        \\
                                 \midrule
\multirow{3}{*}{\makecell{Prop. \\ LLM}} 
                                 & GPT-3.5-turbo     & 98.0        & 97.0 \textcolor{red}{(-1.0)}          & 62.7        & 36.4 \textcolor{red}{(-26.3)}       & 67.1       & 42.4 \textcolor{red}{(-24.6)}       \\
                                 & GPT-4-turbo       & 100.0        & 98.0 \textcolor{red}{(-2.0)}          & 79.3        & 61.7 \textcolor{red}{(-17.6)}       & 82.1       & 70.3 \textcolor{red}{(-11.9)}       \\ 
                                 & Claude2.1         & 99.2        & 100.0 \textcolor[rgb]{0,0.6,0}{(0.8)}             & 58.6        & 48.1 \textcolor{red}{(-10.5)}       & 66.0       & 54.5 \textcolor{red}{(-11.5)}       \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Performance of summarization models on three dimenstion in MultiWOZ, comparing their performance with and without redaction. The 'Unredact' and 'Redact' indicate the scores with and without redaction, respectively. 나중에 re-editing한 뒤 수정 예정}
\end{center}
\end{table*}

==> tables/summarization_model_score/before_editing/total_score.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \begin{center}
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.25}
% \footnotesize
% \begin{tabular}{|c|c|cccc|cccc|cccc|}
% \hline
% \multirow{3}{*}{\textbf{Type}} &
%   \multirow{3}{*}{\textbf{Name}} &
%   \multicolumn{4}{c|}{\textbf{Faithfulness}} &
%   \multicolumn{4}{c|}{\textbf{Completeness}} &
%   \multicolumn{4}{c|}{\textbf{Conciseness}} \\ \cline{3-14} 
%  &
%    &
%   \multicolumn{2}{c|}{\textbf{Non-Dial}} &
%   \multicolumn{2}{c|}{\textbf{Dial}} &
%   \multicolumn{2}{c|}{\textbf{Non-Dial}} &
%   \multicolumn{2}{c|}{\textbf{Dial}} &
%   \multicolumn{2}{c|}{\textbf{Non-Dial}} &
%   \multicolumn{2}{c|}{\textbf{Dial}} \\ \cline{3-14} 
%  &
%    &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \multicolumn{1}{c|}{\textbf{Long}} &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \textbf{Long} &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \multicolumn{1}{c|}{\textbf{Long}} &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \textbf{Long} &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \multicolumn{1}{c|}{\textbf{Long}} &
%   \multicolumn{1}{c|}{\textbf{Short}} &
%   \textbf{Long} \\ \hline
% \multirow{2}{*}{\makecell{Non \\ LLM}} &
%   BART-large &
%   \multicolumn{1}{c|}{91.5} &
%   \multicolumn{1}{c|}{89.5} &
%   \multicolumn{1}{c|}{80.3} &
%   77.9 &
%   \multicolumn{1}{c|}{68.0} &
%   \multicolumn{1}{c|}{16.3} &
%   \multicolumn{1}{c|}{41.9} &
%   31.2 &
%   \multicolumn{1}{c|}{88.1} &
%   \multicolumn{1}{c|}{60.7} &
%   \multicolumn{1}{c|}{79.0} &
%   74.0 \\ \cline{2-14} 
%  &
%   Flan-T5-large &
%   \multicolumn{1}{c|}{84.7} &
%   \multicolumn{1}{c|}{83.3} &
%   \multicolumn{1}{c|}{66.0} &
%   75.4 &
%   \multicolumn{1}{c|}{44.9} &
%   \multicolumn{1}{c|}{16.6} &
%   \multicolumn{1}{c|}{39.8} &
%   32.6 &
%   \multicolumn{1}{c|}{83.8} &
%   \multicolumn{1}{c|}{69.4} &
%   \multicolumn{1}{c|}{70.7} &
%   68.4 \\ \hline
% \multirow{4}{*}{\makecell{Open \\ Source \\ LLM}} &
%   Phi-2 &
%   \multicolumn{1}{c|}{81.8} &
%   \multicolumn{1}{c|}{84.5} &
%   \multicolumn{1}{c|}{83.6} &
%   81.2 &
%   \multicolumn{1}{c|}{56.6} &
%   \multicolumn{1}{c|}{16.9} &
%   \multicolumn{1}{c|}{30.4} &
%   25.6 &
%   \multicolumn{1}{c|}{72.2} &
%   \multicolumn{1}{c|}{43.1} &
%   \multicolumn{1}{c|}{51.1} &
%   50.5 \\ \cline{2-14} 
%  &
%   Mistral-7B-Inst &
%   \multicolumn{1}{c|}{94.7} &
%   \multicolumn{1}{c|}{96.9} &
%   \multicolumn{1}{c|}{91.4} &
%   92.9 &
%   \multicolumn{1}{c|}{77.7} &
%   \multicolumn{1}{c|}{43.1} &
%   \multicolumn{1}{c|}{63.5} &
%   59.7 &
%   \multicolumn{1}{c|}{89.3} &
%   \multicolumn{1}{c|}{70.8} &
%   \multicolumn{1}{c|}{76.9} &
%   76.7 \\ \cline{2-14} 
%  &
%   Llama2-13B-Chat &
%   \multicolumn{1}{c|}{92.7} &
%   \multicolumn{1}{c|}{92.4} &
%   \multicolumn{1}{c|}{91.0} &
%   86.7 &
%   \multicolumn{1}{c|}{63.6} &
%   \multicolumn{1}{c|}{29.3} &
%   \multicolumn{1}{c|}{37.2} &
%   35.8 &
%   \multicolumn{1}{c|}{93.0} &
%   \multicolumn{1}{c|}{64.0} &
%   \multicolumn{1}{c|}{73.0} &
%   73.1 \\ \cline{2-14} 
%  &
%   Mixtral-8x7B-Inst &
%   \multicolumn{1}{c|}{97.4} &
%   \multicolumn{1}{c|}{97.0} &
%   \multicolumn{1}{c|}{98.3} &
%   \textbf{95.6} &
%   \multicolumn{1}{c|}{\textbf{80.5}} &
%   \multicolumn{1}{c|}{\textbf{44.5}} &
%   \multicolumn{1}{c|}{66.8} &
%   60.9 &
%   \multicolumn{1}{c|}{86.9} &
%   \multicolumn{1}{c|}{64.5} &
%   \multicolumn{1}{c|}{76.3} &
%   76.0 \\ \hline
% \multirow{3}{*}{\makecell{Prop. \\ LLM}} &
%   GPT-3.5-turbo &
%   \multicolumn{1}{c|}{95.0} &
%   \multicolumn{1}{c|}{97.2} &
%   \multicolumn{1}{c|}{\textbf{99.0}} &
%   93.8 &
%   \multicolumn{1}{c|}{72.5} &
%   \multicolumn{1}{c|}{42.5} &
%   \multicolumn{1}{c|}{54.6} &
%   50.0 &
%   \multicolumn{1}{c|}{\textbf{92.5}} &
%   \multicolumn{1}{c|}{81.5} &
%   \multicolumn{1}{c|}{70.8} &
%   80.5 \\ \cline{2-14} 
%  &
%   GPT-4-turbo &
%   \multicolumn{1}{c|}{97.3} &
%   \multicolumn{1}{c|}{98.1} &
%   \multicolumn{1}{c|}{98.0} &
%   92.6 &
%   \multicolumn{1}{c|}{78.6} &
%   \multicolumn{1}{c|}{45.0} &
%   \multicolumn{1}{c|}{\textbf{71.3}} &
%   \textbf{64.2} &
%   \multicolumn{1}{c|}{92.4} &
%   \multicolumn{1}{c|}{\textbf{84.3}} &
%   \multicolumn{1}{c|}{\textbf{83.0}} &
%   83.3 \\ \cline{2-14} 
%  &
%   Claude2.1 &
%   \multicolumn{1}{c|}{\textbf{99.3}} &
%   \multicolumn{1}{c|}{\textbf{99.3}} &
%   \multicolumn{1}{c|}{97.6} &
%   95.5 &
%   \multicolumn{1}{c|}{65.0} &
%   \multicolumn{1}{c|}{34.0} &
%   \multicolumn{1}{c|}{56.7} &
%   45.2 &
%   \multicolumn{1}{c|}{85.4} &
%   \multicolumn{1}{c|}{78.0} &
%   \multicolumn{1}{c|}{71.6} &
%   \textbf{85.8} \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{center}
% \end{table*}

==> tables/summarization_model_score/prompt_comparision_table.tex <==
% \begin{table}[]
% % \footnotesize
% \begin{center}
% \setlength{\tabcolsep}{12pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{cccc}
% \Xhline{3\arrayrulewidth}
% \textbf{Prompt} & \textbf{Faith.} & \textbf{Comp.}  & \textbf{Con.} \\ 
% \Xhline{3\arrayrulewidth}
% Default         & 0.921           & \textbf{0.674} & 0.715 \\ \midrule
% CoD             & 0.820           & 0.391          & 0.614          \\
% Ex-Abs          & \textbf{0.971}  & 0.576 & \textbf{0.722} \\
% SummIt          & 0.965           & 0.592          & 0.681          \\ 
% \Xhline{3\arrayrulewidth}
% \end{tabular}
% \caption{Results for prompts (캡션 나중에 상황보고 쓰기)}
% \label{tab:prompt_score}
% \end{center}
% \end{table}

\begin{table}[!t]
\footnotesize
% \captionsetup{skip=2pt}
\begin{center}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\tabcolsep}{5pt} % Adjust the space between columns
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{cccc}
\toprule
Prompt & Faithfulness & Completeness  & Conciseness \\ 
\cmidrule{1-4}
Default & 92.1            & 67.4           & 79.3           \\
\midrule
CoD     & 82.0 \textcolor{red}{(-10.1)}           & 38.7 \textcolor{red}{(-28.7)}           & 69.5 \textcolor{red}{(-9.8)}           \\
Ext-Abs  & 97.1 \textcolor[rgb]{0,0.6,0}{(+5.0)}           & 55.4 \textcolor{red}{(-12.0)}           & 76.4 \textcolor{red}{(-2.9)}           \\
SummIt  & 96.5 \textcolor[rgb]{0,0.6,0}{(+4.4)}           & 56.0 \textcolor{red}{(-11.4)}           & 73.9 \textcolor{red}{(-5.4)}   \\
\bottomrule
\end{tabular}
\vspace*{-0.2cm}
\caption{Impact of prompt engineering using GPT-4-turbo on meeting dialogue (source: MeetingBank). The IAA for fact verification and key-fact alignment is 0.52, 0.51, respectively.}
\label{tab:prompt_score}
\end{center}
\vspace*{-0.5cm}
\end{table}
